Estimating Uncertainty in Landslide Segmentation Models

Landslides are a recurring, widespread hazard. Preparation and mitigation efforts can be aided by a high-quality, large-scale dataset that covers global at-risk areas. Such a dataset currently does not exist and is impossible to construct manually. Recent automated efforts focus on deep learning models for landslide segmentation (pixel labeling) from satellite imagery. However, it is also important to characterize the uncertainty or confidence levels of such segmentations. Accurate and robust uncertainty estimates can enable low-cost (in terms of manual labor) oversight of auto-generated landslide databases to resolve errors, identify hard negative examples, and increase the size of labeled training data. In this paper, we evaluate several methods for assessing pixel-level uncertainty of the segmentation. Three methods that do not require architectural changes were compared, including Pre-Threshold activations, Monte-Carlo Dropout and Test-Time Augmentation -- a method that measures the robustness of predictions in the face of data augmentation. Experimentally, the quality of the latter method was consistently higher than the others across a variety of models and metrics in our dataset.

==> datapreprocess.tex <==

Satellite images collected from Google Earth have different aspect ratios. Convolutional neural networks could be trained using images with multiple aspect ratios with an intermediate global average pooling layer \cite{lin2013network} or spatial pyramid pooling layer \cite{he2015spatial} before convolution layers. However, for uniformity in the comparative study, we reshaped the images to the shape 512 x 512 x 3 using the inter-area interpolation option of OpenCV library\cite{opencv_library}. 

A data annotation tool called LabelMe\cite{labelme2016} was used to label the landslide areas in a satellite image. Data was annotated using images with original dimensions (before reshaping). The tool stores the labels as JSON files. These files were parsed to extract pixel-level information to generate binary masks. The Ground truth binary masks were stored in a separate files as  gray-scale images with reshaped dimensions of 512 x 512 and pixel intensities being either 0 or 1. Intensity values of zero represent non-landslide pixels (background) and intensity values of one represent landslide pixels (foreground). 

We added random data augmentations for two purposes. First, data augmentations are known to improve performance of deep learning models by desensitizing the networks to perturbations that should not matter. More importantly, however, data augmentations also help us avoid unintentionally biased data. For instance, the satellite images extracted from Google Earth were predominantly centered around landslides. Thus, we used random horizontal and vertical translations to avoid this bias. Augmentations also helped the models become more robust to other data quality issues. For instance, due to the low saliency of landslide areas in satellite images, the number of foreground pixels are smaller when compared to typical semantic segmentation tasks. Hence, there is an inherent class-wise imbalance in the dataset. Also, multiple landslide images have cloud cover, which leads to lower visibility of features useful for distinguishing landslide areas in images. Cloud cover can occur in 3 types of scenarios: (1)  pre-event images but not the corresponding post-event images, (2)  post-event images but not their pre-event images, (3) both pre-event and post-event images. How is cloud cover solved using data augmentations? To alleviate the above mentioned problems, the random augmentations included horizontal, vertical and diagonal flips, rotations, translations and Gaussian blurs on satellite images. 

Except Gaussian blurs, other augmentations were applied to corresponding ground truth labels. This resulted in 1092 augmented images used for training our models.   



==> training.tex <==
We trained our network on 1092 paired (pre-event, post-event) images and evaluate on 97 test pairs. LandslideNET was trained with an initial learning rate of $1e^{-4}$ for the first 30 epochs with a batch size of 6 on an NVIDIA RTX 2080 Ti GPU cluster with 16GB of memory. Data pre-processing is carried out before training as mentioned in Section \ref{sec:datapreprocess}. Learning rate is scheduled to decrease with every 20 epochs until $1e^{-9}$. We train the model for a total of 200 epochs. The model takes 1 to 1.5 hours to train. The problem is formulated as a pixel-wise binary classification with a sigmoid activation as the last activation layer since the output data is in the range of [0, 1]. Binary Cross Entropy (BCE) is used as the loss function along with Adam optimizer for supervision. The problem is formulated as a regression with a sigmoid activation layer as the last activation layer since the output data is in the range [0, 1]. A threshold of 0.5 is applied over the prediction mask to generate a binary mask of \{0,1\}. The predicted binary mask is used to classify each pixel as landslide (1) or not-landslide (0).


